QAIR: Practical Query-efficient Black-Box Attacks for Image Retrieval

We study the query-based attack against image retrieval to evaluate its robustness against adversarial examples under the black-box setting, where the adversary only has query access to the top-k ranked unlabeled images from the database. Compared with query attacks in image classification, which produce adversaries according to the returned labels or confidence score, the challenge becomes even more prominent due to the difficulty in quantifying the attack effectiveness on the partial retrieved list. In this paper, we make the first attempt in Query-based Attack against Image Retrieval (QAIR), to completely subvert the top-k retrieval results. Specifically, a new relevance-based loss is designed to quantify the attack effects by measuring the set similarity on the top-k retrieval results before and after attacks and guide the gradient optimization. To further boost the attack efficiency, a recursive model stealing method is proposed to acquire transferable priors on the target model and generate the prior-guided gradients. Comprehensive experiments show that the proposed attack achieves a high attack success rate with few queries against the image retrieval systems under the black-box setting. The attack evaluations on the real-world visual search engine show that it successfully deceives a commercial system such as Bing Visual Search with 98% attack success rate by only 33 queries on average.

==> latex/intro.tex <==

% \begin{table}[h]
%   \centering
%   \footnotesize
%  \setlength{\tabcolsep}{1.5mm}{
%   \begin{tabular}{ l|lll}
%   \toprule[1.5pt]
%          & White box    & Transfer-base & Query-based   \\ \hline
% Required & Target model & Training data & Query access  \\ \hline
% Classification       & FGSM, PGD    & FGSM transfer & BA, HSJA, RGF \\
% Retrieval            & UAP, ODFA    & DeepMisR      & $\bigstar$ Ours \\
%   \hline
%   \toprule[1.5pt]
%   \end{tabular} 
%   }
%     \caption{Taxonomy of adversarial attack methods. Different from existing attacks for image retrieval, our attack is applicable to real-world scenarios because it only needs query access to target model.}
%   \label{tbl:model2}
% \end{table}


% \begin{figure}[h]        
%   \center{\includegraphics[width=1.0\linewidth]{latex/figures/6.png}}
%  \caption{\label{fig:diff_cls_ret} (Left)Taxonomy of adversarial attacks. Different from existing attacks for image retrieval, our attack is applicable to real-world scenarios since it only needs query access to target model. (Right)The output of image classification model(Cls) is a label or confidence score while it is a list of unlabeled images for image retrieval(Ret).}
%  \end{figure}

\begin{figure}[t]        
  \center{\includegraphics[width=1.0\linewidth]{latex/figures/query_Compressed.pdf}}
 \caption{\label{fig:diff_cls_ret_2} 
 (a) (Left)Taxonomy of adversarial attacks. Different from existing attacks for image retrieval(IR), our attack is applicable to real-world scenarios since it only needs query access to target model. (Right)The output of image classification(Cls) is label or confidence score while it is a list of unlabeled images in IR.\\
 (b)Demonstration of the query-based black-box attack on image retrieval(IR) system. Given a black-box model, the attackers use queries to update and generate adversarial perturbations.}
 \end{figure}

Despite of its impressive performance in many tasks such as image classification, object detection and image retrieval, Deep Neural Network~(DNN) has shown its vulnerability to adversarial examples that can trigger the misbehavior with imperceptible perturbations~\cite{goodfellow2014explaining, cheng2019improving}.
Such vulnerability has raised great concerns about the robustness and real-world deployment of DNNs for image retrieval~\cite{li2019universal} and object detection~\cite{chen2018shapeshifter}.
For example, on e-commercial platforms, sellers can steal others' graphic designs and prevent the stolen images from being detected by the retrieval-based copy detection by adding adversarial perturbations.
Therefore, it is crucial to develop a practical robustness evaluation technology to further explore the vulnerability of retrieval systems against adversarial attacks in reality and then develop corresponding countermeasures.

In general, the goal for adversarial attack against image retrieval is to completely subvert the top-$k$ retrieval results. For a practical attack, two important characteristic are required.
\begin{itemize}
\item \textbf{Black-box setting}. In reality, neither the model parameter nor training data is available, making the target model a black-box for attackers. The adversary only has query access to the target model. Besides, the unlabeled retrieved images make it a decision-based problem, where only the attack is successful or not is provided.

\item \textbf{Limited queries}. Too many queries may cost much time and money. Besides, the attack can be easily defended by limiting query times. Thus, a practical attack should require as fewer queries as possible.
\end{itemize}


However, as shown in Fig.~\ref{fig:diff_cls_ret_2}, existing studies on image retrieval attacks are mostly focused on white-box attacks~\cite{zhou2020adversarial, li2019universal,wang2020transferable,shan2020fawkes}.
The underlying assumption on complete knowledge about the model parameters or training data usually does not hold in real-world scenario.
Though some work also evaluate their transfer attacks in black-box way, which attacks the target model by leveraging adversarial examples generated against the white-box substitute models~\cite{wang2020transferable, li2019universal}.
They usually require training data for substitute models, which is not practical in reality.
% It requires large ensembles of substitute models to approximate the target model to maximize the attack success rate. Such attacks can be easily defended once a defender manages to reduce the transferability~\cite{brunner2019guessing}.
Thus, the robustness of image retrieval systems under realistic scenarios leaves to be explored.

In comparison, query-based attacks~\cite{chen2017zoo, narodytska2016simple} generate adversarial examples based on the model output queried from the target model, which are easier to be rendered in real-world situation. 
They can be categorized into score-based attacks and decision-based attacks~\cite{brendel2017decision}.
The latter one is more challenging since attackers can only get the final decision that whether the attack is successful while the former one is aware of  
how much the target model has been attacked with confidence score.
% The former usually needs fewer queries with confidence score that can indicate how much the target model has been attacked while the latter can only get access to whether the attack is successful during attacks.

Though lots of efforts have been devoted in image classification tasks,
existing query-based attacks cannot be directly applied to image retrieval systems as a practical attack.
% There are two main reasons. 
On the one hand, decision-based attacks usually require a tremendous number of queries to perform a successful attack, which is not practical in reality.
On the other hand, as shown in Fig.~\ref{fig:diff_cls_ret_2}, compared to image classification whose output is a label or confidence score that can be used directly to evaluate the attack effect, the output of image retrieval system is usually a list of unlabeled images, making it a decision-based problem. Thus, the output of image retrieval system needs to be further processed to make it measurable.
% It makes the attack effectiveness on retrieval system hard to be quantified, which provides little information to boost the attack algorithms. Thus, score-based methods are restricted.

% For black-box attacks, existing methods can be divided into transfer-based and query-based attacks. 
% The transfer-based attacks~\cite{li2019universal} usually attack the target model by leveraging adversarial examples generated against the white-box substitute models~\cite{wang2020transferable}.
% It requires large ensembles of substitute models to approximate the target model to maximize the attack success rate. Such attacks can be easily defended once a defender manages to reduce the transferability~\cite{brunner2019guessing}.

To address the aforementioned challenges, we introduce the first attempt on practical query-efficient black-box attack against image retrieval.
First of all, we formulate the problem of black-box attacks on image retrieval systems, and propose a new relevance-based loss to quantify the attack effects on target models via detailed probability analysis. In this way, score-based query-attacks in classification can be applied to image retrieval tasks.
% To address the aforementioned challenges, we make the first attempt to quantify the retrieval attack effects by measuring the set similarity on the top-$k$ retrieval results before and after attack.
% First of all, a new relevance-based loss is designed to guide the optimization of adversaries via detailed probability analysis.
Besides, considering the fact that retrieved images are ranked based on similarities with the input image, which can generate plenty of labeled triplets,
a single-image-based model stealing method is proposed to approximate the target model for estimating more accurate gradients during attacks.
% A single-query-based model stealing method is proposed to generate a substitute model for target model, which can help to estimate a more accurate gradient given the target model during attacks. 
Extensive experiments show that the proposed method can achieve high attack success rate against the image retrieval models with a remarkable Recall@$K$ drop. We also evaluate our attack efficacy on real visual search system\footnote{https://www.bing.com/visualsearch\label{bing}}, which demonstrates its practicability in real-world scenario.

% The major contributions of our paper include:
Our main contributions can be summarized as follows:
\begin{itemize}
\item We formulate the problem of query-based black-box attacks against image retrieval systems, and propose a new relevance-based loss to make the attack effects on the target image retrieval models quantifiable.
% \item We make the first attempt to quantify the retrieval attack effects by measuring the set similarity on the top-$k$ retrieval results before and after attack. Accordingly, a new relevance-based loss is designed to guide the optimization of adversaries.
% \item We develop a single-image-based model stealing method to better estimate the gradient of the target model and boost the attack efficiency in a data-free manner.
\item We develop a single-image-based model stealing method to generate a transfer-based prior to boost the query-attack efficiency in a data-free manner.
\item We demonstrate the efficacy of our attack through extensive experiments on simulated environment and real-world commercial system.
% \item Experiments on simulated environment and real-world commercial system demonstrate the effectiveness of our query-based attacking method. 
\end{itemize}

% that real-world visual search engine is vulnerable to adversaries even without the prior knowledge about the target model.

==> latex/intro_2.tex <==

\begin{figure}[t]        
  \center{\includegraphics[width=1.0\linewidth]{latex/figures/9.png}}
 \caption{\label{fig:diff_cls_ret_2} 
 (a) (Left)Taxonomy of adversarial attacks. Different from existing attacks for image retrieval(IR), our attack is applicable to real-world scenarios since it only needs query access to target model. (Right)The output of image classification(Cls) is label or confidence score while it is a list of unlabeled images in IR.\\
 (b)Demonstration of the query-based black-box attack on image retrieval(IR) system. Given a black-box model, the attackers use queries to update and generate adversarial perturbations.}
 \end{figure}

With recent great success of deep neural
networks(DNN) in computer vision, image retrieval(IR) systems based on deep metric learning have been applied to various
tasks, including Google Image Search, PaiLiTao, Digital Rights Management(DRM) etc. 
For example, DRM protects original graphic designs by checking if there is a similar design in the top-$k$ retrieved images with IR systems. However, DNN has shown its vulnerability to adversarial examples that can trigger the misbehavior with imperceptible perturbations recently~\cite{goodfellow2014explaining, cheng2019improving}.
By adding adversarial perturbations on the original image, sellers can subvert the top$k$ images and make the target IR system to retrieve some irrelevant images, which may fool the auditor.
Therefore, it is crucial to develop a practical robustness evaluation technology to further explore the vulnerability of retrieval systems against adversarial attacks in reality and then develop corresponding countermeasures.

% In general, the goal for adversarial attack against image retrieval is to completely subvert the top-$k$ retrieval results. 
To simulate the real attack from outsiders, two important characteristics are required to ensure the practicality for an attack.
\begin{itemize}
\item \textbf{Black-box setting}. In reality, neither the model parameter nor training data is available, making the target model a black-box for attackers. The adversary only has query access to the target model. Besides, the unlabeled retrieved images make it a decision-based problem, where only the attack is successful or not is provided.

\item \textbf{Limited queries}. Too many queries may cost much time and money. Besides, the attack can be easily defended by limiting query times. Thus, a practical attack should require as fewer queries as possible.
\end{itemize}

However, as shown in Fig.~\ref{fig:diff_cls_ret_2}, existing studies on image retrieval attacks are mostly focused on white-box attacks~\cite{zhou2020adversarial, li2019universal,wang2020transferable,shan2020fawkes}.
The underlying assumption on complete knowledge about the model parameters or training data usually does not hold in real-world scenario.
Though some work also evaluate their transfer attacks in black-box way, which attacks the target model by leveraging adversarial examples generated against the white-box substitute models~\cite{wang2020transferable, li2019universal}.
They usually require training data for substitute models, which is not practical in reality.
% It requires large ensembles of substitute models to approximate the target model to maximize the attack success rate. Such attacks can be easily defended once a defender manages to reduce the transferability~\cite{brunner2019guessing}.
Thus, the robustness of image retrieval systems under realistic scenarios leaves to be explored.

In comparison, query-based attacks~\cite{chen2017zoo, narodytska2016simple} generate adversarial examples based on the model output queried from the target model, which are easier to be rendered in real-world situation. 
They can be categorized into score-based attacks and decision-based attacks~\cite{brendel2017decision}.
The latter one is more challenging since attackers can only get the final decision that whether the attack is successful while the former one is aware of  
how much the target model has been attacked with confidence score.
% The former usually needs fewer queries with confidence score that can indicate how much the target model has been attacked while the latter can only get access to whether the attack is successful during attacks.

Though lots of efforts have been devoted in image classification tasks,
existing query-based attacks cannot be directly applied to image retrieval systems as a practical attack.
% There are two main reasons. 
On the one hand, decision-based attacks usually require a tremendous number of queries to perform a successful attack, which is not practical in reality.
On the other hand, as shown in Fig.~\ref{fig:diff_cls_ret_2}, compared to image classification whose output is a label or confidence score that can be used directly to evaluate the attack effect, the output of image retrieval system is usually a list of unlabeled images, making it a decision-based problem. Thus, the output of image retrieval system needs to be further processed to make it measurable.
% It makes the attack effectiveness on retrieval system hard to be quantified, which provides little information to boost the attack algorithms. Thus, score-based methods are restricted.

% For black-box attacks, existing methods can be divided into transfer-based and query-based attacks. 
% The transfer-based attacks~\cite{li2019universal} usually attack the target model by leveraging adversarial examples generated against the white-box substitute models~\cite{wang2020transferable}.
% It requires large ensembles of substitute models to approximate the target model to maximize the attack success rate. Such attacks can be easily defended once a defender manages to reduce the transferability~\cite{brunner2019guessing}.

To address the aforementioned challenges, we introduce the first attempt on practical query-efficient black-box attack against image retrieval.
First of all, we formulate the problem of black-box attacks on image retrieval systems, and propose a new relevance-based loss to quantify the attack effects on target models via detailed probability analysis. In this way, score-based query-attacks in classification can be applied to image retrieval tasks.
% To address the aforementioned challenges, we make the first attempt to quantify the retrieval attack effects by measuring the set similarity on the top-$k$ retrieval results before and after attack.
% First of all, a new relevance-based loss is designed to guide the optimization of adversaries via detailed probability analysis.
Besides, considering the fact that retrieved images are ranked based on similarities with the input image, which can generate plenty of labeled triplets,
a single-image-based model stealing method is proposed to approximate the target model for estimating more accurate gradients during attacks.
% A single-query-based model stealing method is proposed to generate a substitute model for target model, which can help to estimate a more accurate gradient given the target model during attacks. 
Extensive experiments show that the proposed method can achieve high attack success rate against the image retrieval models with a remarkable Recall@$K$ drop. We also evaluate our attack efficacy on real visual search system\footnote{https://www.bing.com/visualsearch\label{bing}}, which demonstrates its practicability in real-world scenario.

% The major contributions of our paper include:
Our main contributions can be summarized as follows:
\begin{itemize}
\item We formulate the problem of query-based black-box attacks against image retrieval systems, and propose a new relevance-based loss to make the attack effects on the target image retrieval models quantifiable.
% \item We make the first attempt to quantify the retrieval attack effects by measuring the set similarity on the top-$k$ retrieval results before and after attack. Accordingly, a new relevance-based loss is designed to guide the optimization of adversaries.
% \item We develop a single-image-based model stealing method to better estimate the gradient of the target model and boost the attack efficiency in a data-free manner.
\item We develop a single-image-based model stealing method to generate a transfer-based prior to boost the query-attack efficiency in a data-free manner.
\item We demonstrate the efficacy of our attack through extensive experiments on simulated environment and real-world commercial system.
% \item Experiments on simulated environment and real-world commercial system demonstrate the effectiveness of our query-based attacking method. 
\end{itemize}

% that real-world visual search engine is vulnerable to adversaries even without the prior knowledge about the target model.

==> latex/intro_3.tex <==

\begin{figure}[t]        
  \center{\includegraphics[width=1.0\linewidth]{latex/figures/query_Compressed.pdf}}
 \caption{\label{fig:diff_cls_ret_2} 
 (a) (Left)Taxonomy of adversarial attacks. Different from existing attacks for image retrieval(IR), our attack is applicable to real-world scenarios since it only needs query access to target model. (Right)The output of image classification(Cls) is label or confidence score while it is a list of unlabeled images in IR.\\
 (b)Demonstration of the query-based black-box attack on image retrieval(IR) system. Given a black-box model, the attackers use queries to update and generate adversarial perturbations.}
 \end{figure}

Despite of its impressive performance in many tasks such as image classification, object detection and image retrieval, 
% \xx{Despite of its impressive performance in many tasks such as image retrieval, a valuable task aiming at finding out images similar to queries from the gallery,}
deep neural network~(DNN) has shown its vulnerability to adversarial examples that can trigger the misbehavior with imperceptible perturbations~\cite{goodfellow2014explaining, cheng2019improving}.
Such vulnerability has raised great concerns about the robustness and real-world deployment of DNNs for image retrieval~\cite{li2019universal} and object detection~\cite{chen2018shapeshifter}.
% For example, on e-commercial platforms, sellers can steal others' graphic designs and prevent the stolen images from being detected by the retrieval-based copy detection by adding adversarial perturbations.
For example, some digital rights managements protect original graphic designs by checking if there exists a same design in the top-$k$ similar ones retrieved from their database. By adding adversarial perturbations on protected designs, attackers can subvert the top-$k$ images and make the target IR system to retrieve some irrelevant images, which may fool the auditor to mistake them for original designs.
Therefore, it is crucial to develop a practical robustness evaluation technology to further explore the vulnerability of DNNs against adversarial attacks in reality and then develop corresponding countermeasures.

Nevertheless, most existing works focus on exploring adversarial samples for image classification models.
Adversarial attacks on image retrieval systems, especially the black-box attacks for simulating realistic scenarios, have been seldom explored. Indeed, DNN-based image retrieval systems are being increasingly deployed in real-world scenarios, such as Google Image Search\footnote{https://images.google.com/\label{google}}, Pailitao\footnote{https://www.pailitao.com/}, {\it etc.}. Therefore, it is crucial to investigating the adversarial samples for image retrieval.

This paper studies the practical query-based attacks for image retrieval(IR) systems to simulate the real attack from outsiders.
In general, there exist several challenges in conducting
such attack on image retrieval systems. First, neither
the model parameter nor training data is available in reality,
making the target model a black-box for attackers. Second,
as shown in Fig.~\ref{fig:diff_cls_ret_2}, the output of image retrieval system is usually a list of unlabeled images. Compared to image classification whose output is a label or confidence score that can be used directly to evaluate the attack effect, the attack effectiveness on retrieval system is hard to be quantified, which
provides little information to boost the attack algorithms.

However, as shown in Fig.~\ref{fig:diff_cls_ret_2}, existing studies on image retrieval attacks are mostly focused on white-box attacks~\cite{zhou2020adversarial, li2019universal,wang2020transferable,shan2020fawkes}.
The underlying assumption on complete knowledge about the model parameters or training data usually does not hold in real-world scenario.
Though some work also evaluate their transfer attacks in black-box way, which attacks the target model by leveraging adversarial examples generated against the white-box substitute models~\cite{wang2020transferable, li2019universal}.
They usually require training data for substitute models, which is not practical in reality.
% Thus, the robustness of image retrieval systems under realistic scenarios leaves to be explored.

In contrast, query-based attacks~\cite{chen2017zoo, narodytska2016simple} generate adversarial examples based on the model output queried from the target model, which are easier to be rendered in real-world situation.
% The latter one is more challenging since attackers can only get the final decision that whether the attack is successful while the former one is aware of how much the target model has been attacked with confidence score.
However, existing query-based attacks for image classification models, including score and decision-based attacks, cannot be directly applied to image retrieval systems as a practical attack. 
On the one hand, decision-based attacks usually require a tremendous number of queries to perform a successful attack, which is not practical in reality. On the other hand, as shown in Fig.~\ref{fig:diff_cls_ret_2}, compared to image classification whose output is a label or confidence score that can be used directly to evaluate the attack effect, the output of image retrieval system is usually a list of unlabeled images, making it a decision-based problem. Thus, the output of image retrieval system needs to be further processed to make it measurable.

To address the aforementioned challenges, we propose the first attempt on practical \textbf{Q}uery-efficient black-box \textbf{A}ttack against \textbf{I}mage \textbf{R}etrieval(QAIR).
First of all, we formulate the problem of black-box attacks on image retrieval systems, and propose a new relevance-based loss to quantify the attack effects on target models via detailed probability analysis. In this way, score-based query-attacks in classification can be applied to image retrieval tasks.
Besides, considering the fact that retrieved images are ranked based on similarities with the input image, which can generate plenty of labeled triplets,
% a data-free model stealing method is proposed to approximate the target model for estimating more accurate gradients during attacks.
a data-free model stealing method is proposed to acquire transferable priors for boosting the query-attack efficiency via the prior-guided gradient estimation.
Extensive experiments show that the proposed method can achieve high attack success rate against the image retrieval models with a remarkable Recall@$K$ drop. We also evaluate our attack efficacy on real visual search system\footnote{https://www.bing.com/visualsearch\label{bing}}, which demonstrates its practicability in real-world scenario.

% The major contributions of our paper include:
Our main contributions can be summarized as follows:
\begin{itemize}
\item We formulate the problem of query-based black-box attacks against image retrieval systems, and propose a new relevance-based loss to make the attack effects on the target image retrieval models quantifiable.
% \item We make the first attempt to quantify the retrieval attack effects by measuring the set similarity on the top-$k$ retrieval results before and after attack. Accordingly, a new relevance-based loss is designed to guide the optimization of adversaries.
% \item We develop a single-image-based model stealing method to better estimate the gradient of the target model and boost the attack efficiency in a data-free manner.
\item We develop a data-free model stealing method to acquire transferable priors for boosting the query-attack efficiency.
\item We demonstrate the efficacy of our attack through extensive experiments on simulated environment and real-world commercial system.
% \item Experiments on simulated environment and real-world commercial system demonstrate the effectiveness of our query-based attacking method. 
\end{itemize}

% that real-world visual search engine is vulnerable to adversaries even without the prior knowledge about the target model.

==> latex/method_2.tex <==
% In this section, we \jf{elaborate} our attack in detail.
% Firstly, we formulate the problem of attacking image retrieval models, and propose a relevance-based loss to quantify the attack effects via probability-based analysis.
% % In this way, we can relax the hard-label problem and score-based methods can be applied. 
% To further boost the attack efficiency, we propose a single-image-based model stealing method to approximate the gradient of target model in a data-free manner.

% The attack procedure can be found in Alg.~\ref{alg:attack}. Given an input image $x$, the stolen model $f_s$ firstly calculates its gradients in white-box way as the basis for query attack. Then we follow the general pipeline of score-based methods to run the gradient estimation with the proposed relevance-based loss. It will help to find the proper direction for the next iteration. The above steps will be repeated until the adversary $\hat{x}$ can attack the target model successfully.

In this section, we first formulate the problem of attacking image retrieval models under the black-box setting and then elaborate our proposed attack.
As shown in Alg.~\ref{alg:attack},
given an input image $x$, we first conduct a white-box attack on a substitute model $s$ which is acquired with a recursive model stealing method (shown in Fig.~\ref{fig:model_stealing}), to provide the transferable priors for the following query-based attack.
Then, we quantify the attack effects via probability-based analysis with a delicately designed relevance-based loss, 
and do gradient estimation following the basic idea of the score-based methods, aiming to provide the proper direction for the attack.
Finally, we repeat the aforementioned steps till the generated adversarial image $\hat{x}$ can deceive the target model successfully.



\subsection{Problem Formulation}
\label{sec:problem_formulation}

% Let $f(x): \mathcal{X} \to \mathbb{R}^d$ denote a metric learning model that extracts extracts a fixed length feature representation in $\mathbb{R}^d$ for an input image $x \in \mathcal{X} \subset \mathbb{R}^n$. Denote $\mathcal{D}_f(x, x_i)=\lVert f(x) - f(x_i) \lVert^2_2$ as the metric that measures the feature distance between two images.
As shown in Fig.~\ref{fig:diff_cls_ret_2}, given a query image $x$, the image retrieval system with metric learning model $f$ and gallery \textbf{G} returns a list of images 
\begin{equation}
    \small{ \texttt{RList}}^n (x, f) = \{x_1, x_2, ..., x_i, ..., x_n | x_i\in\bm{G} \},
\end{equation}
ordered by their similarities to $x$, where $n$ is the number of returned images
% and $f$ projects the query image $x$ to latent feature space as $f(x)$.
and $f$ projects $x$ to the feature space as $f(x)$.
In other words, $\mathcal{D}_f(x, x_i) \leq \mathcal{D}_f(x, x_j), s.t. \, i<j$ where $\mathcal{D}_f(x, x_i)=\lVert f(x) - f(x_i) \lVert^2_2$ is the metric that measures the feature distance between two images.

% We assume that the target model behaves well and the returned images are well organized according to the similarities with input image. 
% Then, the attack goal is to fool the target model into outputting a list of images whose top-$k$ has no overlap with original outputs.
In this paper, the adversary aims to fool the target model into outputting a list of images whose top-$k$ has no overlap with original outputs under the assumption that the target model behaves well, i.e., the returned images are well organized according to the similarities to the input image.
Then, the attack goal can be formalized as
% Hence, the goal can be formally defined as:
% \begin{equation}
% \mathcal{G}^F_{\mathcal{K}}(x) \cap \mathcal{G}^F_{\mathcal{K}}(x+\delta) = \O,  \quad s.t.\quad {||\delta||}_p \leq \epsilon,
% \label{eq:def}
% \end{equation}
\begin{equation}
\small{\texttt{RList}}^{\mathcal{K}}(x, f) \cap 
\small{\texttt{RList}}^{\mathcal{K}}(x+\delta, f) = \O  \quad s.t. \quad {||\delta||}_p \leq \epsilon ,
\label{eq:def}
\end{equation}
% where $\mathcal{K}$ and $\epsilon$ are the number of top-ranked images to be considered and perturbation budget, respectively.
where $\mathcal{K}$ is the number of top-ranked images to be considered and $\epsilon$ is the perturbation budget.

% The above goal can be solved with hard-label-based attacks in query-attacking classifiers~\cite{chen2020hopskipjumpattack}, where only the final decision(top-1 predicted label) instead of probability outputs is available to attackers.
The above goal can be solved by borrowing the idea of decision-based attacks proposed in the image classification task~\cite{chen2020hopskipjumpattack}, in which only the final decision (i.e., the predicted top label) instead of class probabilities is available to attackers.
However, as shown in Fig.~\ref{fig:landscape}(left), the loss landscape is discontinuous, it hence requires combinatorial optimization or exhaustive search algorithms, which may need a tremendous number of queries to perform a successful attack~\cite{cheng2018query}.



% \begin{algorithm}[htb]
% \SetAlgoLined
% % \begin{algorithmic}[1]
% \KwInput{Target model $f$; input image $x$;  stolen model $s$; number of iterations for momentum $N_i$; max number of queries $T$; max perturbation $\epsilon$; step size $\sigma$; learning rate $\alpha$; number of considered images $\mathcal{K}$;}
% \KwOutput{The adversarial example $\hat{x}$.}

% \State Initialize $\hat{x} \gets x, \mathcal{L}^{\text{prev}} \gets 1.0, y \gets \small{\texttt{RList}}^{\mathcal{K}}(x, f)$ 

% \For{$t \gets 1$ to $T/2$}{
%  \State \textit{\{Calculate basis $u$ with stolen model $s$\}} \Comment{Eq.~\ref{eq:MIM}}
%     \State Initialize $\hat{x}^t  \gets \hat{x}, u \gets 0$
    
%     \For{$i \gets 1 $ to $N_i$}{
%     \State $u = \beta \cdot u + \nabla_{\hat{x}^t}(\mathcal{L}_\text{w}(\hat{x}^{t}, y))$
%     \State $\hat{x}^t = \textsc{clip}_{x,\epsilon}(\hat{x}^t + \alpha \cdot \text{sign}(u))$
%     }
 
%     \State \textit{\{Query attack with the resulted basis $u$\}} \Comment{Eq.~\ref{eq:RGF}}
%     % \begin{large}
%     \State $\hat{g} \gets \frac{\mathcal{L}(\hat{x}+\sigma u, y) - \mathcal{L}(\hat{x}, y)}{\sigma} \cdot u$ 
%     %   \end{large}
%     \State $\hat{x} \gets \textsc{clip}_{x,\epsilon}(\hat{x} + \alpha \cdot {\rm{sign}}(\hat{g}))$
%     % \Comment{Eq.~\ref{eq:update}}
    
%     \If {$\mathcal{L}(\hat{x}, y) == \mathcal{L}^{\text{prev}}$}{
%         \State $\sigma \gets 2 \cdot \sigma$ }
%     \State  $\mathcal{L}^{\text{prev}} \gets \mathcal{L}(\hat{x}, y)$
 
%  }
% %  \Return { $l_{\theta}$}
%  \Return Adversarial sample $\hat{x}$
% %  \end{algorithmic}
%  \caption{\label{alg:attack} The query-based attack for image retrieval}
% \end{algorithm}



\begin{algorithm}[t!]
% \small
% \setstretch{1.25}
  \caption{\label{alg:attack} The query-based attack for image retrieval}
%   \begin{spacing}{1.2}
  \begin{algorithmic}[1]
    \Require{Target model $f$; input image $x$;  stolen model $s$; number of iterations for momentum $N_i$; max number of queries $T$; max perturbation $\epsilon$; step size $\sigma$; learning rate $\alpha$; number of considered images $\mathcal{K}$;}
    \State Initialize $\hat{x} \gets x, \mathcal{L}^{\text{prev}} \gets 1.0, y \gets \small{\texttt{RList}}^{\mathcal{K}}(x, f)$ 
    \For{$t \gets 1$ to $T/2$}
    % \State Calculate basis $u$ with $f_s, \hat{x}, y$ \Comment{Eq.~\ref{eq:gradient}}
    \State \textit{\{Calculate basis $u$ with stolen model $s$\}} \Comment{Eq.~\ref{eq:MIM}}
    \State Initialize $\hat{x}^t  \gets \hat{x}, u \gets 0$
    \For{$i \gets 1 $ to $N_i$}
    % \State $u = \beta \cdot u + \text{sign}(\frac{\partial \mathcal{L}_\text{w}(\Hat{x}^{\text{tmp}}, y)}{\partial \Hat{x}^{\text{tmp}}})$
    \State $u = \beta \cdot u + \nabla_{\hat{x}^t}(\mathcal{L}_\text{w}(\hat{x}^{t}, y))$
    \State $\hat{x}^t = \textsc{clip}_{x,\epsilon}(\hat{x}^t + \alpha \cdot \text{sign}(u))$
    \EndFor
    \State \textit{\{Query attack with the resulted basis $u$\}} \Comment{Eq.~\ref{eq:RGF}}
    % \begin{large}
    \State $\hat{g} \gets \frac{\mathcal{L}(\hat{x}+\sigma u, y) - \mathcal{L}(\hat{x}, y)}{\sigma} \cdot u$ 
    %   \end{large}
    \State $\hat{x} \gets \textsc{clip}_{x,\epsilon}(\hat{x} + \alpha \cdot {\rm{sign}}(\hat{g}))$
    \If {$\mathcal{L}(\hat{x}, y) == \mathcal{L}^{\text{prev}}$}
        \State $\sigma \gets 2 \cdot \sigma$
    \EndIf
    \State  $\mathcal{L}^{\text{prev}} \gets \mathcal{L}(\hat{x}, y)$
    \EndFor \\
\Return adversarial sample $\hat{x}$
  \end{algorithmic}
%   \end{spacing}
% \vspace{-1mm}
\end{algorithm}



\subsection{Objective Function}
\label{sec:loss}
% To solve the above problem, we propose to quantify the attack effects on image retrieval model to guide the generation of adversaries. 
% In this way, score-based attacks in image classification can be facilitated to retrieval tasks.
To solve the above problems, we delicately design an objective function to quantify the attack effects on the retrieval model to guide the generation of adversarial images.
Concretely, denote by $P(\hat{x}, y)$ the probability that the adversarial image $\hat{x}$ generated from the input $x$ fails to trigger the target model $f$ to misbehave, and denote by $y$ the true label of $x$, {\it i.e.}, $y=\small{\texttt{RList}}^{\mathcal{K}}(x, f)$.
Then, the objective is
\begin{align}
    {\rm{min}} \,\, \mathcal{L}(\hat{x}, y) = P(\hat{x}, y), \,\, s.t. \,\, ||\delta||_p \leq \epsilon.
\end{align}
% where the constraint is designed for keeping $x$ and $\hat{x}$ close in the input space.


To make $P(\hat{x}, y)$ computable, density estimation methods such as kernel density estimators~\cite{parzen1962estimation} can be applied. 
Since the computation cost is directly related to the number of samples, we need to sample as few samples as possible but approximate the distribution of $x$ as accurately as possible. 
% We use nearest neighbor density estimation method with the $\mathcal{K}$ nearest neighbors of $x$ provided by querying target model. Then:
We leverage the nearest neighbor density estimation method to approximate $P(\hat{x}, y)$ based on the top-$\mathcal{K}$ nearest neighbors of $x$ obtained by querying the target model.
Then, $P(\hat{x}, y)$ can be approximately rewritten as
\begin{eqnarray}
\footnotesize
\label{eqn:entropy}
    P(\hat{x}, y) \approx \sum_{i=1}^\mathcal{K}{P(x_i) P(\hat{x}, y | x_i)} = \sum_{i=1}^\mathcal{K}{\omega_i \cdot \varphi_i},
\end{eqnarray}
where $\omega_i=P(x_i)$ denotes the prior sampling probability and $\varphi_i=P(\hat{x}, y|x_i)$ denotes the conditioned attack failure probability.
% For simplicity, we use $\omega_i=P(g_i^F(x))$ and $y_i=P(x, \hat{x} | g_i^F(x))$ to denote the 
% prior sampling probability and conditioned attack failure probability respectively.


\begin{figure}[!t]
 \center{\includegraphics[width=1.0\linewidth]{latex/figures/loss_landscape_Compressed.pdf}}
 \caption{\label{fig:landscape} Loss ($z$-axis) landscape visualization of the target retrieval model. Compared with perturbations with Gaussian ($x$-axis), the loss gets to 0 faster with adversarial perturbations ($y$-axis), showing the model's vulnerability against adversarial examples.
 We can find the hard-label problem is relaxed from left to middle. When relevance is considered, the loss gets to 0 with smaller perturbations.}
 \end{figure}
 
 
In the typical image retrieval system, $x_i$ is related to $x$ with a specific similarity score. However, this score cannot be obtained under the black-box setting.
% Under black-box setting, 
% One way is treating each $x_i$ equally and $\forall i \in [1,\mathcal{K}], \omega_i = 1/\mathcal{K}$ (\jf{denoted} as \textbf{Count-based Loss}). 
The simplest strategy to tackle this problem is to treat each $x_i$ equally, i.e., $\forall i \in [1,\mathcal{K}], \omega_i = 1/\mathcal{K}$ (denoted as the \textbf{Count-based Loss}).
However, this is not the optimal strategy since it cannot reflect the attack effect in a fine-grained manner.
% Despite of its simplicity, this strategy is not optimal.
% Recall that $x_i$ is related to $x$ by their similarity, we can use the ranking information to approximate the relevance. 
Recall that $x_i$ is ranked according to its similarity to $x$, thus we can use the ranking information to approximate their relevance.
Specifically, we refer to the Normalized Discounted Cumulative Gain metric~(NDCG) used in classical ranking
problem~\cite{jarvelin2017ir} and define $r_i$ as the relevance between $x_i$ and $x$. The probability $P(x_i)$ is defined as:
\begin{equation}
P(x_i) = \omega_i =
\frac{{2^{r_i}-1}}{\sum\nolimits_{i=1}^{\mathcal{K}}({2^{r_i}-1})}.
\label{eq:omega}
\end{equation}
With $r_i=\mathcal{K}-i$, the probability of the $i$-th result to be sampled is
a decaying exponential.

% As to $P(\hat{x}\approx x|g_i^F(x);F)$, it exhibits quite different characteristics. Since the
% gallery set $\bm{G}$ are not attacked, similar gallery images are close to each
% other in the feature space. For a successful attack $\hat{x}$ of $x$, it rarely
% happens that any of $g_i^F(x)$ appears in the search results of $\hat{x}$. In
% other words, if $g_i^F(x)$ appears int the top-k results of $\hat{x}$, near
% neighbors of $g_i^F(x)$ as well as $x$ should also appear, resulting in a
% failure attack. Consequently, we define $\omega_i$ as:
% \begin{equation}
%   \omega_i = \begin{cases}
%       \frac{1}{K}, \quad g_i^F(x) \in \mathcal{G}_n^F(\hat{x}), \\
%       0, \quad g_i^F(x) \not\in \mathcal{G}_n^F(\hat{x})
%     \end{cases}
% \end{equation}

$\varphi_i = P(\hat{x}, y|x_i)$ indicates the attack failure probability of $\hat{x}$ given $x_i$. It can be obtained from the retrieved results. 
If $x_i \in \small{\texttt{RList}}^{\mathcal{K}}(\hat{x}, f)$, both $x$ and $\hat{x}$ are similar to $x_i$ and thus $\hat{x}$ should be similar to $x$, which also means the attack fails.
% Taking the aforementioned rank-sensitive relevance into consideration, suppose $x_i$ ranks at the $j$-th position in $\small{\texttt{RList}}^{\mathcal{K}}(\hat{x}, f)$, then
Considering the aforementioned rank-sensitive relevance and supposing that $x_i$ ranks at the $j$-th position in $\small{\texttt{RList}}^{\mathcal{K}}(\hat{x}, f)$, $\varphi_i$ can be denoted as 
% Consequently,
\begin{equation}
\small
  \varphi_i = \begin{cases}
      \omega_j, \quad x_i \in \small{\texttt{RList}}^{\mathcal{K}}(\hat{x}, f) \,\,{\rm{and}}\,\, x_i=\hat{x}_j \\
      0, \quad x_i \not\in \small{\texttt{RList}}^{\mathcal{K}}(\hat{x}, f)
    \end{cases} .
\end{equation}
% In the end, the final relevance-based objective function $\mathcal{L}$ is:

Then, the \textbf{Relevance-based} objective function $\mathcal{L}$ is rewritten as
 \begin{equation} \label{eq:loss}
     \mathcal{L}(\hat{x}, y) = \sum\nolimits_{i=1}^{\mathcal{K}}\omega_i \cdot
     {\varphi_i}, \,\, s.t. \,\, \|\delta\|_p \leq \epsilon.
    %  \label{eq:final_obj}
 \end{equation}

In this way, the attack effects can be evaluated only based on $\small{\texttt{RList}}^{\mathcal{K}}(x, f)$ and $\small{\texttt{RList}}^{\mathcal{K}}(\hat{x}, f)$ according to Eq.~\ref{eq:loss}.
As shown in Fig.~\ref{fig:landscape}, compared to the count-based loss, the attack with relevance-based loss requires a smaller perturbation to reduce the loss to 0.
% When $\mathcal{G}^F_{\mathcal{K}}(x) \cap \mathcal{G}^F_{\mathcal{K}}(x+\delta) = \O$, we have $\forall i \in [1,\mathcal{K}], g_i^F(x) \not\in \mathcal{G}_\mathcal{K}^F(\hat{x})$. Thus $\mathcal{L}(\hat{x}, \mathcal{G}^F_\mathcal{K}(x))=0$, indicating the consistency between attacking goal and the proposed objective function.


% \subsection{The Whole Pipeline}


 
\subsection{Attack Optimization}
% \textbf{Gradient estimation with transfer-based basis}
Since the decision-based problem in Eq.~\ref{eq:def} is relaxed with the proposed relevance-based loss, 
most of the query-based attacks proposed in image classification tasks can be extended to the retrieval tasks.
% most query-based attacks in classification can be transferred to image retrieval tasks. 
% We \jf{adopt} RGF-attack~\cite{nesterov2017random}
% as our base framework and define its loss as the proposed relevance-based loss to extend it to retrieval systems.
We therefore adopt RGF-attack~\cite{nesterov2017random} as our base framework and define its loss by the proposed relevance-based loss for the extension to retrieval systems.
The attack process can be summarized into two parts, {\it i.e.} gradient estimation and perturbation optimization.  
Denote $u_i$ as the $i$-th sampled basis vector which is sampled for $q$ times and $\hat{g}$ as the final estimated gradient. Then, gradient estimation and perturbation optimization are accomplished as follows:
\begin{equation}
\small
\begin{split}
    \hat{g} = \frac{1}{q}\sum_{i=1}^{q}\hat{g}_i, \,
    \hat{g}_i &= \frac{\mathcal{L}(x+\sigma u_i, y) - \mathcal{L}(x, y)}{\sigma} \cdot u_i, \\
    \hat{x} &= \textsc{clip}_{x,\epsilon}(x + \alpha \cdot {\rm{sign}}(\hat{g})),
\end{split}
\label{eq:RGF}        
\end{equation}
where $\sigma$ is the parameter to control the sampling variance and $\alpha$ is the learning rate.
The $\textsc{clip}_{x,\epsilon}$ operation aims to make the perturbation bounded in the budget~\cite{shi2019curls}. Besides, the generated adversarial example is converted to integer before it is fed into the target model to ensure its validity.



\subsection{Model Stealing for Transferable Priors}
\label{sec:model_stealing}
\xx{In RGF, the basis is randomly sampled due to the lack of knowledge about the target model, resulting in a tremendous number of queries for a successful attack.} For this, some studies have proposed to utilize surrogate models to generate transferable priors for the basis initialization and improve the attack efficiency under the black-box setting~\cite{brunner2019guessing, cheng2019improving}. 
Accordingly, some image retrieval attack methods train a substitute model with the training datasets to mimic the black-box model~\cite{wang2020transferable, li2019universal}. However, training data is unavailable for attackers in reality.
To tackle this problem, we propose to steal the gallery data of the image retrieval system via query access in a recursive manner.

\textbf{Recursive model stealing.}
As shown in Fig.~\ref{fig:model_stealing}, queried by input image $x$, the image retrieval system returns a set of retrieved images $\small{\texttt{RList}}^{n}(x, f)$, from which we select $N_c$ images evenly for greater diversity. 
% Compared to collecting images from websites directly, we can ensure that the gained images are in-distribution of model gallery.
These images again form a new image set as new queries to find more samples.
The above procedure will be repeated for $C$ times to guarantee the diversity of collected images.

According to the principle of image retrieval, retrieved images are ranked by their similarities to the input image. 
Thus, with the collected $M$ images, we can query the target models to get final triplets as the ground-truth for training the surrogate model $s$, of which the objective function is defined as
\begin{equation}
\small
    \sum\nolimits_{j>i} {\left[ \mathcal{D}_s(x, x_i) - \mathcal{D}_s(x, x_j) + \lambda \right]}_{+}.
    \label{eq:mse}
\end{equation}

We set $n=1000$, $N_c=10$, $C=3$ and $\lambda=0.05$ for all experiments. Thus, we only need 1111~(summed by 1+10+100+1000) queries to steal a model. 
Besides, the stolen model is dependent exclusively on the target model.
In addition to the stolen model, the stealing cost is also shared by all the test samples.
For example, the average query cost for each one is only $1 \approx 1111/1000$ if the number of test samples is 1000.

Our model stealing method features a great advantage that 
it needs no data beforehand.
This is quite different from model distillation  algorithms~\cite{li2019universal} which is usually performed based on the same training data with the target model.
It also differs from generative model based methods~\cite{zhou2020dast} , in which the collected data are usually out-of-distribution from the galleries of the target model. 
Besides, the diversity of the generated samples may be limited due to the problem of mode collapse.
In contrast, by querying target models constantly, we can steal data from the gallery in a recursive manner and guarantee the performance.



\begin{figure}[!t]        
  \center{\includegraphics[width=1.0\linewidth]{latex/figures/steal_Compressed.pdf}}
 \caption{\label{fig:model_stealing} The pipeline of our model stealing. First, an arbitrary image is put into the target image retrieval (IR) system (\textcircled{1}). The retrieved images are then evenly selected to construct a new query set, which will be put into the IR system in the next iteration ($\textcircled{2}, \textcircled{3}$) for more triplets. Finally, The stolen triplets ($\textcircled{4}$) will be used to train the substitute model $s$.}
 \end{figure}


\begin{figure*}[htb]        
 \center{\includegraphics[width=1.0\linewidth]{latex/figures/result_Compressed.pdf}}
 \vspace{-3mm}
 \caption{\label{fig:result_procedure} Visualization of the attack procedures (left) and attack results (right). Images in red boxes are generated adversarial examples, which can fool the target model to return irrelevant images with imperceptible perturbations in the corresponding rows. Scores on the left are the corresponding loss to their searched results on their right. As more samples in the original sets disappear, the loss decays to 0.}
 \vspace{-4mm}
 \end{figure*}



\begin{table*}[h]
\renewcommand\arraystretch{1.2}
  \centering
  \footnotesize
%   \scriptsize
 \setlength{\tabcolsep}{0.65mm}{
   \begin{tabular}{ c|cccccc|c|c|cccc|c|c|cccccc|c|c  }
   \toprule[1.2pt]
    \multirow{2}*{Attacks} &  \multicolumn{8}{c|}{CUB-200}  & \multicolumn{6}{c|}{SOP} & \multicolumn{8}{c}{In-Shop}  \\ \cline{2-23}
 	~ & 1  & 2 & 4 & 8 & 16 & 32 & AQ & ASR & 1 & 10 & 100 & 1000 & AQ & ASR & 1  & 10 & 20 & 30 & 40 & 50 & AQ & ASR\\
 	\hline
 	 	\hline
 	 Original & 
%  	 0.73 & 0.81 & 0.87 & 0.91 & 0.95 & 0.99 & 0 & 0
 	 0.61 & 0.73 & 0.87 & 0.91 & 0.98 & 0.99 & 0 & 0
 	 & 0.724 & 0.816 & 0.904 & 0.960 & 0 & 0
 	 & 0.642 & 0.868 & 0.910 & 0.926 & 0.938 & 0.945 & 0 & 0
 	  \\ \hline\hline
 	 \multicolumn{23}{c}{Comparsion with the State-of-the-art Methods}\\ \hline\hline
 	 OptAttack~\cite{cheng2018query} &
 	 \textbf{0.08} & \textbf{0.15} & \textbf{0.30} & 0.49 & 0.63 & 0.89 & 9708 & 0.04
 	 & 0.012 & 0.032 & 0.744 & 0.928 & 7931 & 0.288
 	 & \textbf{0.004} & \textbf{0.020} & 0.564 & 0.680 & 0.764 & 0.828 & 3017 & \textbf{0.948}
 	 \\
 	 
 	 Sign-Opt~\cite{cheng2019sign} &
 	 0.11 & 0.21 & 0.35 & 0.57 & 0.70 & 0.88 & 8833 & 0.00
 	 & 0.008 & 0.024 & 0.696 & 0.916 & 6746 & 0.372
 	 & 0.014 & 0.032 & 0.464 & 0.560 & 0.660 & 0.728 & 5564 & 0.492
 	 \\
 	 
 	 HSJA~\cite{chen2020hopskipjumpattack} & 
 	 0.13 & 0.23 & 0.41 & 0.47 & 0.60 & 0.92 & 10000 & 0.00
 	 & \textbf{0} & \textbf{0} & 0.632 & 0.880 & 5888 & 0.420
 	 & 0.004 & 0.024 & 0.316 & 0.470 & 0.564 & 0.624 & 5379 & 0.472\\
 	 \hline
 	 
 	 QAIR &
 	 0.16 & 0.23 & 0.32 & \textbf{0.45} & \textbf{0.56} & \textbf{0.76} & \textbf{93} & \textbf{0.69}
 	 & 0.016 & 0.064 & \textbf{0.472} & \textbf{0.832} & \textbf{35} & \textbf{0.904}
 	 & 0.008 & 0.044 & \textbf{0.132} & \textbf{0.256} & \textbf{0.312} & \textbf{0.352} & \textbf{35} & 0.916
 	 \\ \hline\hline
 	 
 	 \multicolumn{23}{c}{Component Analysis}\\ \hline\hline
 	 
 	 C-QAIR &
 	 0.59 & 0.76 & 0.83 & 0.94 & 0.96 & 0.97 & 199 & 0.01
 	 & 0.176 & 0.372 & 0.724 & 0.916 & 113 & 0.480
 	 & 0.296 & 0.556 & 0.716 & 0.764 & 0.800 & 0.832 & 147 & 0.310
 	  \\ 
 	 C-QAIR-I &
 	 0.36 & 0.51 &  0.60  &  0.74 & 0.80 & 0.92 & 152 & 0.32
 	 & 0.060 & 0.112 & 0.572 & 0.868 & 60 & 0.812
 	 & 0.072 & 0.164 & 0.272 & 0.396 & 0.476 & 0.520 & 65 & 0.784
 	  \\
 	 C-QAIR-S &
 	 0.31 & 0.46 & 0.52 & 0.58 & 0.72 & 0.85 & 142 & 0.37
 	 & 0.056 & 0.088 & 0.532 & 0.848 & 51 & 0.836
 	 & 0.052 & 0.124 & 0.204 & 0.320 & 0.404 & 0.432 & 50 & 0.844
 	  \\ 
%  	 R-QAIR-S &
%  	 0.27 & 0.35 & 0.46 & 0.54 & 0.70 & 0.83 & 119 & 0.56
%  	 & 0.028 & 0.080 & 0.516 & 0.868 & 45 & 0.876
%  	 & 0.028 & 0.100 & 0.196 & 0.292 & 0.368 & 0.440 & 40 & 0.880
%  	  \\ 
 	  
 	  \hline
 	  
   R-QAIR-S &
 	 \textbf{0.16} & \textbf{0.23} & \textbf{0.32} & \textbf{0.45} & \textbf{0.56} & \textbf{0.76} & \textbf{93} & \textbf{0.69}
 	 & \textbf{0.016} & \textbf{0.064} & \textbf{0.472} & \textbf{0.832} & \textbf{35} & \textbf{0.904}
 	 & \textbf{0.008} & \textbf{0.044} & \textbf{0.132} & \textbf{0.256} & \textbf{0.312} & \textbf{0.352} & \textbf{35} & \textbf{0.916} \\
 	\hline
   \toprule[1.2pt]
   \end{tabular} 
   }
%   \vspace{-2mm}
    \caption{
    Comparison with state-of-the-art methods on CUB-200, SOP and In-Shop before (Original) and after attack (others). Smaller Recall@K, smaller average number of queries (AQ) over both successful and failed attacks as well as higher Attack Success Rate (ASR) mean stronger attack.
    }
  \label{tbl:result}
  \vspace{-2mm}
\end{table*}
 

\textbf{Transferable priors.}
\xx{With the stolen model, which can generate transferable priors for boosting the attack efficiency}, we follow the state-of-the art work Learnable Black-Box Attack~\cite{yang2020learning}, which utilizes the surrogate model $s$ to guide the basis selection.
Specifically, Momentum Iterative Method (MIM)~\cite{dong2018boosting} is firstly adopted to conduct the white-box attack based on the stolen model.
The derived momentum item $u$ is then used as the basis for the query-based attack. 
The loss $\mathcal{L}_\text{w}$ used for white-box attack is
\begin{equation}
\small
\mathcal{L}_\text{w}(\hat{x}, y) = ||s(\hat{x}) - \sum\nolimits_{i=1}^{\mathcal{K}} w_i \cdot s (x_i)||^2_2.
\label{eq:mse}
\end{equation}


And the optimization procedure for momentum is:
\begin{equation}
    \begin{split}
    u &= \beta \cdot u + \nabla_{\hat{x}}(\mathcal{L}_\text{w}(\hat{x}, y)), \\
    \hat{x} &= \textsc{clip}_{x,\epsilon}(\hat{x} + \alpha \cdot \text{sign}(u)),
    \end{split}
\label{eq:MIM}
\end{equation}
where $u$ is initialized with $\boldsymbol{0}$ and $\beta = 0.9$. The above procedure will be repeated for $N_i$ times. 

The whole attack procedure can be found in Alg.~\ref{alg:attack}. Note that our QAIR is different from previous transfer-based attacks against image retrieval that utilize substitute models for crafting adversarial examples directly. Instead, QAIR employs the stolen model for obtaining transferable priors and generating prior-guided gradients for query attack. In this way, adversarial examples can be further rectified with query response until the attack succeeds.



==> latex/related.tex <==

% Adversarial attack has raised great concerns about the robustness of DNNs since it can deceive DNN models with imperceptible perturbations~\cite{goodfellow2014explaining}. As a more operable adversarial attack, the query-based attack is the greatest threat since it only requires black-box access to the output of the target models~\cite{brendel2017decision}. However, such attack has not been studied on image retrieval systems. 
% In this section, we briefly review adversarial examples and attacks for image retrieval as well as the typical query-based attacks for image classification.
In this section, we first briefly review adversarial attacks in the context of image classification and then introduce some related work in image retrieval.

% \subsection{Adversarial Attack}
\subsection{Query-based Adversarial Attack}
Adversarial examples are maliciously crafted by adding human-imperceptible perturbations that trigger DNNs to misbehave~\cite{goodfellow2014explaining}. 
The attacks for generating adversarial examples can be summarized into gradient-based attack~\cite{goodfellow2014explaining,madry2017towards}, transfer-based attack~\cite{dong2020benchmarking} and  query-based attack~\cite{brendel2017decision,chen2020hopskipjumpattack} in terms of the model information that attackers rely on during attack.
The query-based attack is more practical since the adversary in reality usually only has query access to the output of the target model and does not have any detailed information about model gradient or training data.
This kind of attack has been widely studied in the task of image classification and can be primarily divided into score-based attack and decision-based attack. 

\textbf{Score-based.} 
% Score-based attacks need fewer queries with more information(the confidence score)~\cite{chen2017zoo, nesterov2017random}.
Under this setting, attackers have access to the confidence score of the prediction, which can help to indicate the process of attack~\cite{chen2017zoo, nesterov2017random}.
Most score-based attacks usually estimate the gradient by zero-order optimization methods through query access to the output of the target model~\cite{cheng2019improving}. 
Specifically, a perturbation is firstly initialized and added to the input image. The output score will guide the algorithm to find out the optimization direction of the next step.
% The key issues of such attacks are the adversarial objective function and gradient estimation. The latter one guides the generation of perturbations while the former one determines whether the disturbation is effective.
% For score-based scenario in classification, the confidence scores  can be directly treated as the guidance.
% Hence, the main challenge is how to estimate the gradients based on the defined loss.
% To this end, 
For instance, Zeroth Order Optimization Based Black-box Attack(Zoo)~\cite{chen2017zoo} estimates the gradient at each coordinate by using the symmetric difference quotient.  
To improve the query efficiency, a random gradient-free(RGF) method~\cite{nesterov2017random} is proposed to get approximated gradient by
sampling random vectors independently from a distribution.
% For example, random gradient-free(RGF) method~\cite{nesterov2017random} gets approximated gradient by sampling random vectors from a distribution for $q$ times as bases to improve the query efficiency. 
% In RGF-attack, the optimization process can be divided into two parts, {\it i.e.}, basis initialization and gradient estimation. The basis initialization is achieved by sampling random vectors independently from a distribution $\mathcal{P}$ for $q$ times. 
% Denote $u_i$ as the $i$-th sampled basis vector and $\hat{g}$ as the final estimated gradient. Then gradient estimation is accomplished as follows:
% \begin{equation}
% \small
%     \hat{g} = \frac{1}{q}\sum_{i=1}^{q}\hat{g}_i, \,
%     \hat{g}_i = \frac{\mathcal{L}(x+\sigma u_i, y) - \mathcal{L}(x, y)}{\sigma} \cdot u_i,
%     \label{eq:RGF}
% \end{equation}
% where $y$ is the true label of $x$, $\sigma$ is a parameter to control the sampling variance and  $\mathcal{L}$ is the loss function, for example, cross entropy loss in RGF.
% % We set $q=1$, $\sigma=0.1$ for all experiments.
% With the estimated gradient, the adversary can be optimized as:
% \begin{equation}
%     \hat{x} = \textsc{clip}_{x,\epsilon}(x + \alpha * {\rm{sign}}(\hat{g})),
%     \label{eq:update}
% \end{equation}
% where $\alpha$ is the learning rate.
% % and it is set to 0.01 in our experiment. 
% The $\textsc{clip}_{x,\epsilon}$ operation aims to make the perturbation bounded in the budget~\cite{shi2019curls}.
Besides, recent work~\cite{brunner2019guessing, wallace2020imitation} also uses the gradient of a surrogate model to improve the efficiency of black-box attacks. But the training of substitute model requires huge amount of data which may not be obtained in real applications. Though some work~\cite{zhou2020dast, kariyappa2020maze} propose to steal model in a data-free manner, {\it e.g.}, producing inputs by generative models, this issue needs to be further investigated in image retrieval tasks.

\textbf{Decision-based.} Different from score-based ones, attacks under decision-based setting are more challenging since only successful or not is provided.
They usually treat an irrelevant or target image as start point and decrease the perturbation gradually to make the adversarial similar to input image in visually during optimization~\cite{brendel2017decision, cheng2019sign, chen2020hopskipjumpattack}. 
For example, Boundary Attack~\cite{brendel2017decision} starts the attack from an image lies in the target class.
At each step, a perturbation is sampled from a proposal distribution, which reduces the distance of the perturbed image towards the original input. If the perturbed image still lies in the target class, the perturbation is kept. Otherwise, the perturbation is dropped. 
High attack success rate as it holds, it requires a tremendous number of queries to achieve small perturbations.
% Their goal is to find minimum perturbation in limited queries.
% Thus, they usually hold high success rate but require a tremendous number of queries to achieve small perturbations.

% \subsection{Adversarial Examples} 
% % Adversarial examples is a kind of attack that can fool neural networks by images with intentionally imperceptible perturbation.

% Formally, in image classification, given a benign image $x$ and a target model $f$, 
% % the attack goal is generating an adversary $\hat{x}=x+\delta$ that satisfies:
% an adversarial example $\hat{x}$ is generated by adding the imperceptible noise $\delta$ that satisfies:
% \begin{equation}
%     f(x) \neq f(\hat{x}) = f(x+\delta), \,\,s.t.\,\, ||\delta||_p \leq \epsilon,
% \end{equation}
% where $\epsilon$ is the perturbation budget and $p$ determines the kind of matrix/tensor norm (possible choices can be $\ell_1$, $\ell_2$ and $\ell_\infty$) to measure the perturbation. 

% Adversarial attacks can be roughly divided into two categories: white-box such as Fast Gradient Sign Method(FGSM)~\cite{goodfellow2014explaining}, Projected Gradient Descent(PGD)~\cite{madry2017towards} and black-box attacks in terms of whether the model parameters are available for attackers. And black-box attacks can be further divided into transfer-based such as FGSM-transfer~\cite{dong2020benchmarking} and query-based attacks such as Boundary Attack(BA)~\cite{brendel2017decision}, HopSkipJumpAttack(HSJA)~\cite{chen2020hopskipjumpattack} according to if attackers update their adversaries with query results.


\subsection{Adversarial Attacks for Image Retrieval}
Image retrieval is a long-standing research topic in computer vision and it has been widely used in e-commercial systems such as Google Image Searching\textsuperscript{\ref{google}}, Bing Visual Search\textsuperscript{\ref{bing}}, {\it etc.}. A deep metric learning based image retrieval system usually consists of metric learning model and a database or gallery~\cite{wang2019multi}. The former one extracts the feature of input image and find images from the latter in terms of their similarities with input image.

According to the principle of image retrieval, the earliest white-box attack approach for image retrieval models, {\it i.e.}, Opposite Direction Feature Attack~(ODFA)~\cite{zheng2018open} is introduced. ODFA generates adversarial examples by querying target model's parameters and pushing away the feature of adversarial query in the opposite direction of original feature. 
A comprehensive study on white-box adversarial effects in person re-identification named DeepMisRanking~(DeepMisR) is later proposed~\cite{bai2019metric}.

To generate image-agnostic universal adversarial perturbations~(UAP) in image retrieval, Li~{\it et al.}~\cite{li2019universal} propose to break the neighbourhood relationships of image features via degrading corresponding ranking metric. Under the white-box setting, they try to optimize the traditional triplet loss inversely against metric learning on feature embeddings. As for black-box attack, coarse-to-fine rank distillation is proposed to distill target model by regressing ranking list. However, the model architecture is assumed to be known. Besides, model distillation is performed with a subset from training data of target model, which is usually not available in reality. 
Recently, some strategies~\cite{wang2020transferable,zhou2020dast} are proposed to improve the transferability of adversarial examples, but the application is limited by the collection of datasets used to train substitute models.
Thus, query-based attack for image retrieval still needs to be exploited.



